Learning a Sparse Neural Network using IHT

The core of a good model is in its ability to focus only on important information that reflects the basic patterns and consistencies, thus pulling out a clear, noise-free signal from the dataset. This necessitates using a simplified model defined by fewer parameters. The importance of theoretical foundations becomes clear in this context, as this paper relies on established results from the domain of advanced sparse optimization, particularly those addressing nonlinear differentiable functions. The need for such theoretical foundations is further highlighted by the trend that as computational power for training NNs increases, so does the complexity of the models in terms of a higher number of parameters. In practical scenarios, these large models are often simplified to more manageable versions with fewer parameters. Understanding why these simplified models with less number of parameters remain effective raises a crucial question. Understanding why these simplified models with fewer parameters remain effective raises an important question. This leads to the broader question of whether there is a theoretical framework that can clearly explain these empirical observations. Recent developments, such as establishing necessary conditions for the convergence of iterative hard thresholding (IHT) to a sparse local minimum (a sparse method analogous to gradient descent) are promising. The remarkable capacity of the IHT algorithm to accurately identify and learn the locations of nonzero parameters underscores its practical effectiveness and utility. This paper aims to investigate whether the theoretical prerequisites for such convergence are applicable in the realm of neural network (NN) training by providing justification for all the necessary conditions for convergence. Then, these conditions are validated by experiments on a single-layer NN, using the IRIS dataset as a testbed.

==> definitions/bce_loss.tex <==
\begin{definition}[Binary Cross Entropy Loss]\label{def:BCE}
Let $\hat{y} \in [0,1]$ be a predicted probability for a true label whose value is either zero or one, i.e., $y \in \{0,1\}$. The Binary Cross Entropy (BCE) loss is defined as follows:
$$
\text{BCE}(y,\hat{y})
=
-\Big(y \log(\hat{y}) + (1 - y)\log(1 - \hat{y})
\Big).
$$
\end{definition}

==> definitions/cross_entropy_loss.tex <==
\begin{definition}[Cross Entropy Loss]\label{def:CE}
Let $\hat{\mathbf{y}} \in (0,1)^c \in \mathbb{R}^c$ ($c \geq 3$) be a predicted probability for a true one-hot vector label $\mathbf{y} \in \mathbb{R}^c$, i.e., $y_j=1, y_i=0$ for $j\neq i=1, \dots, c$. The Cross Entropy (CE) loss is defined as follows:
$$
\text{CE}(y,\hat{y})
=
-\sum_{i=1}^{c}y_i\log (\hat{y}_i).
$$
\end{definition}

==> definitions/gradient_definition.tex <==
\begin{definition}[Gradient of a scalar-valued function]\label{def:gradient}
Let $f:\mathbb{R} \to \mathbb{R}$ be a differentiable scalar-valued function. The gradient of  $\nabla f: \mathbb{R}^n \to \mathbb{R}^n$ at $\mathbf{x} \in \mathbb{R}^n$ is defined as the following:
$$
\nabla f(\mathbf{x})
=
\begin{bmatrix}
 \frac{\partial f(\mathbf{x})}{\partial x_1}
\\
 \vdots
\\
 \frac{\partial f(\mathbf{x})}{\partial x_n}
 \end{bmatrix}.
$$
\end{definition}

==> definitions/jacobian_definition.tex <==
\begin{definition}[Jacobian matrix of a vector-valued function]\label{def:jacobian}
Let $\mathbf{f}: \mathbb{R}^n \to \mathbb{R}^m$ be a differentiable vector-valued function where 
$
\mathbf{f}(\mathbf{x})
=
\begin{bmatrix}
f_1(\mathbf{x})
\\
\vdots
\\
f_m(\mathbf{x})
\end{bmatrix}
$
 and $\mathbf{x} \in \mathbb{R}^n$. This function takes a point $\mathbf{x} \in \mathbb{R}^n$ as an input and produces $\mathbf{f}(\mathbf{x})\in \mathbb{R}^m$ as the output. The Jacobian matrix of $\mathbf{f}$ with respect to $\mathbf{x}$ is defined to be an $m \times n$ matrix denoted by $\mathbf{J}_{\mathbf{x}} \mathbf{f}(\mathbf{x})$ as the following:
 $$
 \mathbf{J}_{\mathbf{x}} \mathbf{f}(\mathbf{x})
 =
 \begin{bmatrix}
 \frac{\partial f_1(\mathbf{x})}{\partial x_1}
 &
 \cdots
&
 \frac{\partial f_1(\mathbf{x})}{\partial x_n}
 \\
 \vdots
 &
 \ddots
 &
 \vdots
 \\
 \frac{\partial f_m(\mathbf{x})}{\partial x_1}
 &
 \cdots
&
 \frac{\partial f_m(\mathbf{x})}{\partial x_n}
 \end{bmatrix}
 =
 \begin{bmatrix}
 \big(
\nabla_{\mathbf{x}} f_1(\mathbf{x}) 
\big)^{\top} 
\\
\vdots
\\
\big(
\nabla_{\mathbf{x}}
f_m(\mathbf{x})  
\big)^{\top}
 \end{bmatrix}.
 $$
\end{definition}

==> definitions/mse_loss.tex <==
\begin{definition}[Squared Error Loss]\label{def:SE}
Let $\hat{y} \in \mathbb{R}$ be a predicted value for a true label whose value is $y \in \mathbb{R}$. The Square Error (SE) loss is defined as follows:
$$
\text{SE}(y,\hat{y})
=
(y-\hat{y})^2.
$$
\end{definition}

==> definitions/sigmoid_function.tex <==
\begin{definition}[Sigmoid function]\label{def:sigmoid}
A sigmoid function $\sigma: \mathbb{R} \to [0,1]$ is defined as $\sigma(x)=\frac{e^x}{1+e^x}$.
\end{definition}

==> definitions/softmax_function.tex <==
\begin{definition}[Softmax function]\label{def:softmax}
A softmax function $\bm{\sigma}: \mathbb{R}^c \to \mathbb{R}^c$ is defined for $c\geq 3$ as the following:
$$
\bm{\sigma}(\mathbf{x})
=
\begin{bmatrix}
\frac{e^{x_1}}{\sum_{j=1}^{c}e^{x_j}}
\\
\vdots
\\
\frac{e^{x_c}}{\sum_{j=1}^{c}e^{x_j}}
\end{bmatrix}
\in \mathbb{R}^c.
$$
\end{definition}

==> figures/convolution.tex <==
\begin{figure}[t]
    \centering \includegraphics[scale=0.2]{pics/Convolution.pdf}
    \caption{An illustration of convolution}
\label{fig:convolution}
\end{figure}

==> figures/init_support_vs_last_support.tex <==
\begin{figure}[t]
    \centering 
    \includegraphics[scale=0.4]{pics/init_support_vs_last_support.pdf}
    \caption{Initialilzation support vs $k$-th step support}
    \label{fig:initvslast}
\end{figure}

==> figures/iris_sparse_training/iris_sparse_l_hats.tex <==
\begin{figure}
    \centering
    \includegraphics[scale=0.45]{pics/iris_pics/iris_lr.png}
    \caption{Estimated learning rate for all sparsity levels, i.e., $1 \leq s <n=15$.}
    \label{fig:iris-sparse-learning-rate}
\end{figure}

==> figures/iris_sparse_training/iris_test_acc.tex <==
\begin{figure}
    \centering
    \includegraphics[scale=0.45]{pics/testing_accuracy.png}
    \caption{Test accuracy for all sparsity levels, i.e., $1 \leq s <n=15$.}
    \label{fig:iris-test-acc}
\end{figure}

==> figures/iris_sparse_training/iris_test_loss.tex <==
\begin{figure}
    \centering
    \includegraphics[scale=0.45]{pics/testing_loss.png}
    \caption{Test loss for all sparsity levels, i.e., $1 \leq s <n=15$.}
    \label{fig:iris-test-loss}
\end{figure}

==> figures/iris_sparse_training/iris_training_acc.tex <==
\begin{figure}
    \centering
    \includegraphics[scale=0.45]{pics/training_accuracy.png}
    \caption{Training accuracy for all sparsity levels, i.e., $1 \leq s <n=15$.}
    \label{fig:iris-training-acc}
\end{figure}

==> figures/iris_sparse_training/iris_training_loss.tex <==
\begin{figure}
    \centering
    \includegraphics[scale=0.45]{pics/traning_loss.png}
    \caption{Training loss for all sparsity levels, i.e., $1 \leq s <n=15$.}
    \label{fig:iris-training-loss}
\end{figure}

==> figures/last-layer_activation_and_loss_combination.tex <==
\begin{figure}[t]
    \centering 
\includegraphics[scale=0.4]{pics/last-layer_activation_and_loss_combination.pdf}
    \caption{Last-Layer activation function combined with its associated loss}
    \label{fig:activaionllosscombination}
\end{figure}

==> figures/lenet.tex <==
\begin{figure*}[t]
    \centering 
\includegraphics[scale=0.14]{pics/LeNet.pdf}
    \caption{LeNet-100-300-10}
\label{fig:threelayernetwork}
\end{figure*}

==> figures/linearclassifier.tex <==
\begin{figure}[b]
    \centering 
    \includegraphics[scale=0.2]{pics/3-class_classifier_with_4_features.pdf}
    \caption{3-class classifier with 4  features and a single layer.}
    \label{fig:linearclassifier}
\end{figure}


==> figures/one_layer_network.tex <==
\begin{figure}[b]
    \centering 
    \includegraphics[scale=0.16]{pics/3-class_classifier_with_4_features.pdf}
    \caption{3-class classifier with 4  features and a single layer.}
    \label{fig:onelayernetwork}
\end{figure}

==> figures/one_layer_sparse_finalization.tex <==
\begin{figure}
    \centering
    \includegraphics[scale=0.45]{pics/initialization_parameters_s7_trained.png}
    \caption{Trained parameters obtained from the IHT with random initialization, data
and support seeds of 21, 42 and 84.}
    \label{fig:sparse-trained-params}
\end{figure}


==> figures/one_layer_sparse_initialization.tex <==
\begin{figure}
    \centering
    \includegraphics[scale=0.45]{pics/initialization_parameters_s7.png}
    \caption{Sparse initialization with random initialization and support seeds of 21 and 84.}
    \label{fig:init-and-supp-seeds}
\end{figure}


==> figures/separated_last_layer.tex <==
\begin{figure}[b]
    \centering 
    \includegraphics[scale=0.3]{pics/separated_last_layer.pdf}
    \caption{Separating the last layer activation from a DNN}
    \label{fig:separatedLastLayer}
\end{figure}

==> figures/subspaces.tex <==
\begin{figure}[t]
    \centering 
    \includegraphics[scale=0.5]{pics/subspaces.png}
    \caption{Multiple Subspaces in $\mathbb{R}^3$.}
    \label{fig:subspaces}
\end{figure}

==> figures/training.tex <==
\begin{figure}[t]
    \centering 
    \includegraphics[scale=0.3]{pics/training.pdf}
    \caption{Relationship between training of a NN and BP algorithm}
    \label{fig:training}
\end{figure}


==> figures/two_layer_network.tex <==
\begin{figure}[t]
    \centering 
    \includegraphics[scale=0.1]{pics/two_layer_network.pdf}
    \caption{Two-layer network}
    \label{fig:twolayernetwork}
\end{figure}


==> tables/number_of_basic_feasible_points.tex <==
\begin{table*}[t]
\centering
\caption{Number of $n = 15$}
\label{tab:bfpoints}
\scalebox{1}{
\begin{tabular}{@{}l *{14}{c}@{}}
\hline\toprule
Sparsity levels ($s$) 
 & 1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 & 9 & 10 & 11 & 12 & 13 & 14 
\\\midrule
Number of BF points
 & 15 & 105 & 455 & 1,365 & 3,003 & 5,005 & 6,435 & 6,435 & 5,005 & 3,003 & 1,365 & 455 & 105 & 15
\\\midrule
Learning rate
 & 15 & 105 & 455 & 1,365 & 3,003 & 5,005 & 6,435 & 6,435 & 5,005 & 3,003 & 1,365 & 455 & 105 & 15
\\\midrule
Number of HT-stable points
 & 15 & 105 & 455 & 1,365 & 3,003 & 5,005 & 6,435 & 6,435 & 5,005 & 3,003 & 1,365 & 455 & 105 & 15
\\\midrule
Number of HT-unstable points
& 15 & 105 & 455 & 1,365 & 3,003 & 5,005 & 6,435 & 6,435 & 5,005 & 3,003 & 1,365 & 455 & 105 & 15
\\
\bottomrule\hline
\end{tabular}
}
\end{table*}


==> tables/number_of_steps_for_IHT.tex <==
\begin{table*}[t]
\centering
\caption{Number of steps for different sparsity levels}
\label{tab:ihtsteps}
\scalebox{1}{
\begin{tabular}{@{}l *{14}{c}@{}}
\hline\toprule
Sparsity levels ($s$) 
 & 1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 & 9 & 10 & 11 & 12 & 13 & 14 
\\\midrule
Steps
 & 15 & 105 & 455 & 1,365 & 3,003 & 5,005 & 6,435 & 6,435 & 5,005 & 3,003 & 1,365 & 455 & 105 & 15
\\
\bottomrule\hline
\end{tabular}
}
\end{table*}
